Discrete Subgraph Sampling for Interpretable Graph based Visual Question Answering

Explainable artificial intelligence (XAI) aims to make machine learning models more transparent. While many approaches focus on generating explanations post-hoc, interpretable approaches, which generate the explanations intrinsically alongside the predictions, are relatively rare. In this work, we integrate different discrete subset sampling methods into a graph-based visual question answering system to compare their effectiveness in generating interpretable explanatory subgraphs intrinsically. We evaluate the methods on the GQA dataset and show that the integrated methods effectively mitigate the performance trade-off between interpretability and answer accuracy, while also achieving strong co-occurrences between answer and question tokens. Furthermore, we conduct a human evaluation to assess the interpretability of the generated subgraphs using a comparative setting with the extended Bradley-Terry model, showing that the answer and question token co-occurrence metrics strongly correlate with human preferences. Our source code is publicly available.

==> content/related_work.tex <==
\section{Related Work}

\subsection{Visual Question Answering}
Despite the rise of foundational models such as \llava~\cite{llava,improvedllava,llavanext}, \chatgpt~\cite{chatgpt}, \gemini~\cite{gemini}, or \llama~\cite{llama}, the field of \gls{vqa} is still an active area of research.
\citet{bokvqa} proposed a bilingual version of the OK-VQA~\cite{okvqa} dataset and show improvements of pre-training graph emebeddings that can be injected into the \gls{vqa} system.

\subsection{Graph based Visual Question Answering}
\citet{graphvqa} proposed language guided \gls{gnns} for \gls{gvqa} using the ground-truth scene graphs of \gqa.
\citet{tilli} extend the approach by incorporating a discrete subgraph sampling layer into the \gls{gat} to increase the interpretability of the model.

\citet{dsamr} 

\subsection{Interpretable and Explainable GVQA}
Despite the interpretable approach by \citet{tilli}, other works aim to increase the interpretability for such models as well.
\citet{medicalvqa}
\citet{interpretablegraphokvqa}

\subsection{Discrete Sampling}

\subsection{Unified Perspective}
Closest to our work is the work by \citet{tilli} who propose a discrete subgraph sampling layer for \gls{gvqa} within their \gls{gat} model.
However, they focused on one method that intrinsically generates a subgraph along the prediction of the model.
In contrast, we study the effects of different sampling strategies on the model's performance and interpretability.


